A Query Language for Software Architecture Information (Extended version)

Software maintenance is an important part of a software system's life cycle. Maintenance tasks of existing software systems suffer from architecture information that is diverging over time (architectural drift). The Digital Architecture Twin (DArT) can support software maintenance by providing up-to-date architecture information. For this, the DArT gathers such information and co-evolves with a software system, enabling continuous reverse engineering. But the crucial link for stakeholders to retrieve this information is missing. To fill this gap, we contribute the Architecture Information Query Language (AIQL), which enables stakeholders to access up-to-date and tailored architecture information. We derived four application scenarios in the context of continuous reverse engineering. We showed that the AIQL provides the required functionality to formulate queries for the application scenarios and that the language scales for use with real-world software systems. In a user study, stakeholders agreed that the language is easy to understand and assessed its value to the specific stakeholder for the application scenarios.

==> impl.tex <==
% \section{Implementation}
% \label{sec:Impl}
To show the real work applicability of our designed language
we implemented a prototype using the DArT.\footnote{Due to confidentiality reasons as required by our industry partner, the source code cannot be provided, as the concrete language highly depends on the DArT's meta-model.}
For this, we analyzed available tools for model querying and language implementation, 
from which we selected the Epsilon Object Language~\cite{Kolovos2006} and the Xtext language workbench~\cite{Eysholdt2010}.
The implementation enables manual along with automated use cases, 
by providing a query builder API and editing capabilities.
Executing queries via the API returns lists of Java objects,
while using the provided graphical editor and interpreter the results are marshaled into JSON format.
Leveraging code generation through Xtext and a model-to-text transformation, 
the implementation can adapt to changes in the model with low effort,
 resulting in higher maintainability.

